DPMA: Learning to Compress Mixture-of-Experts Models

Mixture-of-Experts (MoE) architectures offer high computational efficiency, but storing all experts requires substantial memory and limits deployment on resource-constrained hardware. Most retraining-free MoE compression methods commit to either pruning or merging experts, often with a uniform compression ratio across layers. We introduce DPMA (Differentiable Prune Merge Absorb), which jointly learns compression operations and layer-wise expert allocation through gradient descent under a global expert budget. Separate learnable coefficients allow DPMA to prune experts, merge their parameters, and absorb their routing contributions by forwarding routing weights to retained experts. These coefficients and expert assignments are optimised to match the original model's outputs on calibration data while its weights remain frozen. Across four MoE models, eight multiple-choice benchmarks, and five compression ratios, DPMA achieves the highest accuracy averaged over benchmarks and compression ratios on each model among the evaluated methods. At $75\%$ expert reduction, it outperforms the strongest baseline on every model, with gains of up to $6.7$ percentage points.

==> preamble_adapter.tex <==
\makeatletter

\def\@paper@title{Untitled}
\let\@paper@titlerunning\@empty
\let\@paper@keywords\@empty
\let\@paper@code\@empty
\let\@paper@plainauthors\@empty
\let\@paper@displayauthors\@empty
\let\@paper@displayaffils\@empty
\let\@paper@corrdisplay\@empty
\let\@paper@titlelogo\@empty
\def\paper@titlelogoheight{3.0em}
\def\paper@titlelogowidth{0.14\linewidth}
\def\paper@titlelogogap{0.03\linewidth}
\def\paper@abstractfile{sections_abstract}
\newcounter{paper@affil}
\let\@neurips@authors\@empty
\let\@neurips@affils\@empty
\let\@neurips@corr\@empty
\let\@mlsys@authors\@empty
\let\@mlsys@affils\@empty
\let\@mlsys@corr\@empty
\newif\if@paper@firstauthor \@paper@firstauthortrue
\newif\if@paper@firstdisplayauthor \@paper@firstdisplayauthortrue
\newif\if@paper@hasequal \@paper@hasequalfalse
\newlength{\paper@titlecardinnerwidth}

\def\paper@titlecardpadding{0.45cm}
\def\paper@titlecardradius{10pt}

\definecolor{paperBrandCamlsysBlue}{HTML}{102344}
\definecolor{paperBrandCambridgeRed}{HTML}{EF2E31}
\definecolor{paperBrandCambridgeGold}{HTML}{FDDD04}
\colorlet{paperTitleBgCamlsys}{paperBrandCamlsysBlue!8!white}
\colorlet{paperTitleBgCambridgeGold}{paperBrandCambridgeGold!8!white}
\colorlet{paperTitleBgCambridge}{paperBrandCambridgeRed!3!paperTitleBgCambridgeGold}
\colorlet{paperTitleBgNeutral}{black!2!white}
\colorlet{paperTitleBg}{paperTitleBgCamlsys}
\definecolor{paperTitleFg}{HTML}{1F2328}
\definecolor{paperTitleMuted}{HTML}{4D5560}
\def\paper@titlebg@camlsys{camlsys}
\def\paper@titlebg@cambridge{cambridge}
\def\paper@titlebg@neutral{neutral}

\csdef{paper@sym@equal}{*}

\newcommand{\paperTitle}[1]{\def\@paper@title{#1}}
\newcommand{\paperKeywords}[1]{\def\@paper@keywords{#1}}
\newcommand{\paperCode}[1]{\def\@paper@code{#1}}
\newcommand{\paperAbstractFile}[1]{\def\paper@abstractfile{#1}}
\newcommand{\paperTitleLogo}[1]{\def\@paper@titlelogo{#1}}
\newcommand{\paperTitleLogoHeight}[1]{\def\paper@titlelogoheight{#1}}
\newcommand{\paperTitleLogoWidth}[1]{\def\paper@titlelogowidth{#1}}
\newcommand{\paperTitleLogoGap}[1]{\def\paper@titlelogogap{#1}}
\newcommand{\paperTitleBackground}[1]{%
  \edef\paper@titlebg@choice{#1}%
  \ifx\paper@titlebg@choice\paper@titlebg@camlsys
    \colorlet{paperTitleBg}{paperTitleBgCamlsys}%
  \else
    \ifx\paper@titlebg@choice\paper@titlebg@cambridge
      \colorlet{paperTitleBg}{paperTitleBgCambridge}%
    \else
      \ifx\paper@titlebg@choice\paper@titlebg@neutral
        \colorlet{paperTitleBg}{paperTitleBgNeutral}%
      \else
        \ClassWarning{paper}{Unknown title-card background theme `\paper@titlebg@choice'; keeping current theme}%
      \fi
    \fi
  \fi
}
\paperTitleBackground{\paper@titlebg}
\newcommand{\paperTitleRunning}[1]{%
  \def\@paper@titlerunning{#1}%
  \ifpaper@mlsys \mlsystitlerunning{#1}\fi  %
}

\newcommand{\addAffiliation}[2]{%
  \stepcounter{paper@affil}%
  \csedef{paper@affil@#1}{\thepaper@affil}%
  \ifnum\value{paper@affil}>\@ne \appto\@paper@displayaffils{\quad}\fi
  \protected@eappto\@paper@displayaffils{\noexpand\textsuperscript{\arabic{paper@affil}}}%
  \appto\@paper@displayaffils{#2}%
  \ifpaper@neurips
    \ifnum\value{paper@affil}>\@ne \appto\@neurips@affils{\quad}\fi
    \protected@eappto\@neurips@affils{\noexpand\textsuperscript{\arabic{paper@affil}}}%
    \appto\@neurips@affils{#2}%
  \fi
  \ifpaper@mlsys
    \appto\@mlsys@affils{\mlsysaffiliation{#1}{#2}}%
  \fi
}

\newcommand{\paper@resolvekey}[1]{%
  \ifcsdef{paper@sym@#1}{%
    \ifstrequal{#1}{equal}{\@paper@hasequaltrue}{}%
    \protected@eappto\@paper@syms{\csuse{paper@sym@#1}}%
  }{%
    \ifcsdef{paper@affil@#1}{%
      \ifx\@paper@nums\@empty\else\appto\@paper@nums{,}\fi
      \protected@eappto\@paper@nums{\csuse{paper@affil@#1}}%
    }{\ClassWarning{paper}{\noexpand\addAuthor: unknown key `#1'}}%
  }%
}
\newcommand{\addAuthor}[2]{%
  \ifx\@paper@plainauthors\@empty
    \appto\@paper@plainauthors{#1}%
  \else
    \appto\@paper@plainauthors{, #1}%
  \fi
  \let\@paper@nums\@empty \let\@paper@syms\@empty
  \forcsvlist{\paper@resolvekey}{#2}%
  \if@paper@firstdisplayauthor\else\appto\@paper@displayauthors{,\space}\fi
  \appto\@paper@displayauthors{#1}%
  \protected@eappto\@paper@displayauthors{\noexpand\textsuperscript{\@paper@nums\@paper@syms}}%
  \@paper@firstdisplayauthorfalse
  \ifpaper@neurips
    \if@paper@firstauthor\else\appto\@neurips@authors{,\space}\fi
    \appto\@neurips@authors{#1}%
    \protected@eappto\@neurips@authors{\noexpand\textsuperscript{\@paper@nums\@paper@syms}}%
    \@paper@firstauthorfalse
  \fi
  \ifpaper@mlsys
    \appto\@mlsys@authors{\mlsysauthor{#1}{#2}}%
  \fi
}

\newcommand{\correspondingAuthor}[2]{%
  \appto\@paper@corrdisplay{#1 \texttt{<#2>}}%
  \ifpaper@neurips \appto\@neurips@corr{\thanks{Correspondence to: #1 \texttt{<#2>}}}\fi
  \ifpaper@mlsys   \appto\@mlsys@corr{\mlsyscorrespondingauthor{#1}{#2}}\fi
}

\newcommand{\paper@setneuripspdfauthor}{%
  \hypersetup{pdfauthor={\@paper@plainauthors}}%
}
\newcommand{\paper@setmlsyspdfauthor}{%
  \hypersetup{pdfauthor={\@paper@plainauthors}}%
}
\newcommand{\paper@setpdfmetadata}{%
  \@ifpackageloaded{hyperref}{%
    \hypersetup{pdftitle={\@paper@title}}%
    \ifx\@paper@keywords\@empty\else
      \hypersetup{pdfkeywords={\@paper@keywords}}%
    \fi
    \ifpaper@neurips
      \paper@setneuripspdfauthor
    \fi
    \ifpaper@mlsys
      \paper@setmlsyspdfauthor
    \fi
  }{}%
}

\newcommand{\paper@titleLogoGraphic}{%
  \IfFileExists{\@paper@titlelogo}{%
    \includegraphics[height=\paper@titlelogoheight,width=\linewidth,keepaspectratio]{\@paper@titlelogo}%
  }{%
    \ClassWarning{paper}{Title logo `\@paper@titlelogo' not found}%
    \fbox{\rule{0pt}{\paper@titlelogoheight}\textsf{\small logo}}%
  }%
}

\newcommand{\paper@titleLine}{%
  \ifx\@paper@titlelogo\@empty
    {\raggedright\sffamily\bfseries\huge\color{paperTitleFg}\@paper@title\par}%
  \else
    \noindent
    \begin{minipage}[c]{\paper@titlelogowidth}
      \centering\paper@titleLogoGraphic
    \end{minipage}\hspace{\paper@titlelogogap}%
    \begin{minipage}[c]{\dimexpr\linewidth-\paper@titlelogowidth-\paper@titlelogogap\relax}
      {\raggedright\sffamily\bfseries\huge\color{paperTitleFg}\@paper@title\par}%
    \end{minipage}\par
  \fi
}

\newcommand{\paper@identityBlock}{%
  \ifx\@paper@displayauthors\@empty\else
    {\sffamily\bfseries\small\color{paperTitleFg}%
      \exhyphenpenalty=0\looseness=-1\@paper@displayauthors\par}%
  \fi
  \ifx\@paper@displayaffils\@empty\else
    \vspace{0.10cm}%
    {\small\color{paperTitleMuted}\@paper@displayaffils\par}%
  \fi
}

\newcommand{\paper@metadataText}{%
  \if@paper@hasequal
    \textsuperscript{*}Equal contribution.\par
  \fi
  \ifx\@paper@corrdisplay\@empty\else
    {\sffamily\bfseries Correspondence:} \@paper@corrdisplay\par
  \fi
  \ifx\@paper@keywords\@empty\else
    {\sffamily\bfseries Keywords:} \@paper@keywords\par
  \fi
  \ifx\@paper@code\@empty\else
    {\sffamily\bfseries Code:} \@paper@code\par
  \fi
}

\newlength{\paper@logostripwidth}
\newcommand{\paper@titlecardlogos}{\paperLogoStrip}
\newcommand{\paper@measureLogoStrip}{%
  \renewcommand{\paper@titlecardlogos}{\paperLogoStrip}%
  \ifx\paper@logos\paper@logos@none
    \setlength{\paper@logostripwidth}{0pt}%
  \else
    \settowidth{\paper@logostripwidth}{\paperLogoStrip}%
  \fi
  \ifdim\paper@logostripwidth>0.52\paper@titlecardinnerwidth
    \renewcommand{\paper@titlecardlogos}{%
      \resizebox{0.52\paper@titlecardinnerwidth}{!}{\paperLogoStrip}}%
    \setlength{\paper@logostripwidth}{0.52\paper@titlecardinnerwidth}%
  \fi
}
\newcommand{\paper@metadataRow}{%
  \noindent
  \begin{minipage}[t]{\dimexpr\linewidth-\paper@logostripwidth-0.25cm\relax}
    {\small\color{paperTitleMuted}\paper@metadataText}%
  \end{minipage}\par
}

\newcommand{\paper@titlecardLogoOverlay}{%
  \ifx\paper@logos\paper@logos@none\else
    \node[
      anchor=south east,
      inner sep=0pt,
      outer sep=0pt,
      xshift=-\paper@titlecardpadding,
      yshift=\paper@titlecardpadding
    ] at (paperTitleCardNode.south east) {\paper@titlecardlogos};%
  \fi
}

\newcommand{\paper@titlecard}{%
  \begingroup
    \setlength{\paper@titlecardinnerwidth}{\dimexpr\linewidth-\paper@titlecardpadding-\paper@titlecardpadding\relax}%
    \paper@measureLogoStrip
    \noindent
    \begin{tikzpicture}
      \node[
        fill=paperTitleBg,
        rounded corners=\paper@titlecardradius,
        inner sep=\paper@titlecardpadding,
        outer sep=0pt,
        text width=\paper@titlecardinnerwidth,
        align=left
      ] (paperTitleCardNode) {%
        \begin{minipage}{\paper@titlecardinnerwidth}
          \setlength{\parindent}{0pt}%
          \setlength{\parskip}{0pt}%
          \raggedright
          \paper@titleLine
          \vspace{0.30cm}%
          \paper@identityBlock
          \vspace{0.38cm}%
          {\small\justifying\color{paperTitleFg}{\sffamily\bfseries Abstract.}\space\input{\paper@abstractfile}\par}%
          \vspace{0.22cm}%
          \paper@metadataRow
        \end{minipage}%
      };%
      \paper@titlecardLogoOverlay
    \end{tikzpicture}%
    \par\vspace{0.35cm}%
  \endgroup
}

\newcommand{\paper@setmlsysrunninghead}{%
  \ifx\@paper@titlerunning\@empty
    \gdef\@mlsystitlerunning{\@paper@title}%
  \else
    \gdef\@mlsystitlerunning{\@paper@titlerunning}%
  \fi
  \chead{\small\bf\@mlsystitlerunning}%
  \thispagestyle{empty}%
}

\newcommand{\makepapertitle}{%
  \paper@setpdfmetadata
  \ifpaper@neurips
    \par
    \begingroup
      \thispagestyle{empty}%
      \paper@titlecard
      \@notice
    \endgroup
  \fi
  \ifpaper@mlsys
    \paper@setmlsysrunninghead
    \twocolumn[%
      \paper@titlecard
      \vskip 0.18in
    ]%
  \fi
}

\makeatother


==> preamble_format.tex <==
\makeatletter

\newif\ifpaper@neurips
\newif\ifpaper@mlsys
\newif\ifpaper@twocolumn

\def\paper@@neurips{neurips}
\def\paper@@mlsys{mlsys}
\ifx\paper@format\paper@@mlsys
  \paper@mlsystrue
\else
  \ifx\paper@format\paper@@neurips
    \paper@neuripstrue
  \else
    \ClassError{paper}{Unknown format `\paper@format'; use format=neurips or format=mlsys}{}%
  \fi
\fi

\ifpaper@neurips
  \paper@twocolumnfalse
  \RequirePackage[preprint]{neurips_2026}%
  \def\paperbibstyle{plainnat}%
\fi

\ifpaper@mlsys
  \paper@twocolumntrue
  \providecommand{\theHalgorithm}{\arabic{algorithm}}%
  \RequirePackage[accepted]{mlsys2026}%
  \def\paperbibstyle{mlsys2026}%
\fi

\makeatother


==> preamble_logos.tex <==
\makeatletter

\newcommand{\paper@logo}[4]{%
  \raisebox{-0.5\height}{%
    \IfFileExists{branding_#1.pdf}{\includegraphics[height=#4,trim=#3,clip]{branding_#1.pdf}}{%
    \IfFileExists{branding_#1.png}{\includegraphics[height=#4]{branding_#1.png}}{%
    \IfFileExists{branding_#1.jpg}{\includegraphics[height=#4]{branding_#1.jpg}}{%
    \fbox{\rule[-1.5mm]{0pt}{#4}\textsf{\scriptsize\,#2\,}}}}}%
  }%
}

\newcommand{\paper@logo@ikerlan}{\paper@logo{ikerlan}{Ikerlan}{17.8bp 18.5bp 17bp 18.5bp}{5.5mm}}
\newcommand{\paper@logo@hitz}{\paper@logo{hitz}{HiTZ}{26bp 82.2bp 26bp 80.1bp}{3.6mm}}
\newcommand{\paper@logo@camlsys}{\paper@logo{camlsys}{CaMLSys}{67bp 67bp 67bp 67bp}{7mm}}
\newcommand{\paper@logo@flower}{\paper@logo{flower}{Flower Labs}{79bp 88.7bp 79bp 89bp}{6.5mm}}
\newcommand{\paper@logo@ucam}{\paper@logo{cambridge}{University of Cambridge}{0bp 0bp 0bp 0bp}{10mm}}
\newcommand{\paper@logo@sofair}{\paper@logo{sofair}{SOFAIR}{0bp 0bp 0bp 0bp}{6mm}}

\def\paper@logos@none{none}
\def\paper@logos@ih{ikerlan-hitz}
\def\paper@logos@ihf{ikerlan-hitz-flower}
\def\paper@logos@ichf{ikerlan-camlsys-hitz-flower}
\def\paper@logos@extended{ikerlan-cambridge-camlsys-sofair-hitz-flower}

\newcommand{\paper@logosep}{\hspace{2mm}}

\newcommand{\paperLogoStrip}{%
  \ifx\paper@logos\paper@logos@none\else
    \begingroup
      \ifx\paper@logos\paper@logos@extended
        \renewcommand{\paper@logosep}{\hspace{0.8mm}}%
        \paper@logo@ikerlan\paper@logosep\paper@logo@ucam\paper@logosep
        \paper@logo@camlsys\paper@logosep\paper@logo@sofair\paper@logosep
        \paper@logo@hitz\paper@logosep
        \paper@logo@flower
      \else
      \ifx\paper@logos\paper@logos@ichf
        \paper@logo@ikerlan\paper@logosep\paper@logo@camlsys\paper@logosep
        \paper@logo@hitz\paper@logosep\paper@logo@flower
      \else
        \ifx\paper@logos\paper@logos@ihf
          \paper@logo@ikerlan\paper@logosep\paper@logo@hitz\paper@logosep
          \paper@logo@flower
        \else
          \paper@logo@ikerlan\paper@logosep\paper@logo@hitz
        \fi
      \fi
      \fi
    \endgroup
  \fi
}

\newcommand{\logoHeader}{%
  \ifx\paper@logos\paper@logos@none\else
    \begin{center}\paperLogoStrip\end{center}%
    \vspace{0.5\baselineskip}%
  \fi
}

\makeatother


==> preamble_macros.tex <==
\makeatletter

\graphicspath{{figures/}{figures/plots/}{figures/diagrams/}{figures/tikz/}{branding_}}

\newenvironment{widefigure}[1][tbp]
  {\ifpaper@twocolumn \@nameuse{figure*}[#1]\else \@nameuse{figure}[#1]\fi}
  {\ifpaper@twocolumn \@nameuse{endfigure*}\else \@nameuse{endfigure}\fi}
\newenvironment{widetable}[1][tbp]
  {\ifpaper@twocolumn \@nameuse{table*}[#1]\else \@nameuse{table}[#1]\fi}
  {\ifpaper@twocolumn \@nameuse{endtable*}\else \@nameuse{endtable}\fi}

\newcommand{\eg}{e.g.,\xspace}
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\etal}{et~al.\xspace}
\newcommand{\dashes}{---\xspace}

\DeclareRobustCommand{\dpma}{\texttt{DPMA}\xspace}
\DeclareRobustCommand{\dpmahard}{\texttt{DPMA\textsubscript{hard}}\xspace}
\DeclareRobustCommand{\dpmasoft}{\texttt{DPMA\textsubscript{soft}}\xspace}
\DeclareRobustCommand{\reap}{\texttt{REAP}\xspace}
\DeclareRobustCommand{\diep}{\texttt{DiEP}\xspace}
\DeclareRobustCommand{\ean}{\texttt{EAN}\xspace}
\DeclareRobustCommand{\naee}{\texttt{NAEE}\xspace}
\DeclareRobustCommand{\eep}{\texttt{EEP}\xspace}
\DeclareRobustCommand{\msmoe}{\texttt{M-SMoE}\xspace}
\DeclareRobustCommand{\hcsmoe}{\texttt{HC-SMoE}\xspace}
\DeclareRobustCommand{\freq}{\texttt{Frequency}\xspace}
\DeclareRobustCommand{\rand}{\texttt{Random}\xspace}

\newcommand{\todo}[1]{{\normalfont\color{red}\,[TODO: #1]\,}}
\newcommand{\note}[2]{{\normalfont\color{blue}\,[#1: #2]\,}}

\makeatother


==> preamble_packages.tex <==
\makeatletter

\RequirePackage{etoolbox}   %

\RequirePackage{iftex}
\ifPDFTeX
  \RequirePackage[utf8]{inputenc}
  \RequirePackage[T1]{fontenc}
\fi

\RequirePackage{graphicx}
\RequirePackage{booktabs}        %
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{amsfonts}
\RequirePackage{mathtools}
\RequirePackage{microtype}
\RequirePackage{xcolor}
\RequirePackage{nicefrac}
\RequirePackage{xspace}
\RequirePackage{siunitx}\sisetup{round-mode=places, round-precision=2}
\RequirePackage{csvsimple}       %
\RequirePackage{pgfplots}\pgfplotsset{compat=1.18}
\RequirePackage{tikz}
\usetikzlibrary{arrows.meta,positioning,shapes.geometric,calc,fit,backgrounds}
\RequirePackage{standalone}      %
\RequirePackage{subcaption}      %

\RequirePackage{algorithm}
\RequirePackage{algorithmic}
\providecommand{\theHalgorithm}{\arabic{algorithm}}

\@ifpackageloaded{hyperref}{}{\RequirePackage{hyperref}}
\definecolor{paperlink}{rgb}{0.10,0.20,0.55}
\hypersetup{colorlinks=true, linkcolor=paperlink, citecolor=paperlink, urlcolor=paperlink, breaklinks=true}
\RequirePackage[capitalise, nameinlink]{cleveref}

\makeatother


==> sections_abstract.tex <==
Mixture-of-Experts (MoE) architectures offer high computational efficiency, but storing all experts requires substantial memory and limits deployment on resource-constrained hardware.
Most retraining-free MoE compression methods commit to either pruning or merging experts, often with a uniform compression ratio across layers.
We introduce \dpma (Differentiable Prune Merge Absorb), which jointly learns compression operations and layer-wise expert allocation through gradient descent under a global expert budget.
Separate learnable coefficients allow \dpma to prune experts, merge their parameters, and absorb their routing contributions by forwarding routing weights to retained experts.
These coefficients and expert assignments are optimized to match the original model's outputs on calibration data while its weights remain frozen.
Across four MoE models, eight multiple-choice benchmarks, and five compression ratios, \dpma achieves the highest accuracy averaged over benchmarks and compression ratios on each model among the evaluated methods.
At $75\%$ expert reduction, it outperforms the strongest baseline on every model, with gains of up to $6.7$ percentage points.

